Cons-free Programs and Complexity Classes between LOGSPACE and PTIME

Programming language concepts are used to give some new perspectives on a long-standing open problem: is logspace = ptime ?

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{L. Fribourg and M. Heizmann (Eds.): VPT/HCVS 2020\\
EPTCS 320, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.320.5}{10.4204/EPTCS.320.5}}

